Privacy- and Utility-Preserving Textual Analysis via Calibrated Multivariate Perturbations

Accurately learning from user data while providing quantifiable privacy guarantees provides an opportunity to build better ML models while maintaining user trust. This paper presents a formal approach to carrying out privacy preserving text perturbation using the notion of dx-privacy designed to achieve geo-indistinguishability in location data. Our approach applies carefully calibrated noise to vector representation of words in a high dimension space as defined by word embedding models. We present a privacy proof that satisfies dx-privacy where the privacy parameter epsilon provides guarantees with respect to a distance metric defined by the word embedding space. We demonstrate how epsilon can be selected by analyzing plausible deniability statistics backed up by large scale analysis on GloVe and fastText embeddings. We conduct privacy audit experiments against 2 baseline models and utility experiments on 3 datasets to demonstrate the tradeoff between privacy and utility for varying values of epsilon on different task types. Our results demonstrate practical utility (< 2% utility loss for training binary classifiers) while providing better privacy guarantees than baseline models.

==> madlib_kdd_appendices.tex <==
\begin{appendices}

\section{Mechanism Pseudo-code}\label{app:madlib}

The following pseudo-code provides implementation details for our text redaction mechanism.
Details about how to sample from the noise distribution $p_N$ can be found in \cite[Appendix E]{wu2017bolt}.

\begin{algorithm}[h]
\DontPrintSemicolon
\SetKw{KwRelease}{release}
\caption{Text Redaction Mechanism}\label{alg:madlib}
\KwIn{string $x_s = w_1 w_2 \cdots w_{\ell}$, privacy parameter $\varepsilon > 0$}
\For{$i \in \{1, \ldots, \ell\}$}{
Compute embedding $\phi_i = \phi(w_i)$\;
Perturb embedding to obtain $\hat{\phi}_i = \phi_i + N$ with noise density $p_N(z) \propto \exp(- \varepsilon \norm{z})$\;
Obtain perturbed word $\hat{w}_i = \argmin_{u \in \cW} \norm{\phi(u) - \hat{\phi}_i}$\;
Insert $\hat{w}_i$ in $i$th position of $\hat{x}_s$\;
}
\KwRelease{$\hat{x}_s$}
\end{algorithm}

\section{Proof of Theorem~\ref{thm:M-mdp}}\label{app:proof}

The intuition behind the proof is to observe that $M$ can be viewed as a combination of the generic exponential mechanism construction for the metric $d$ together with a post-processing strategy that does not affect the privacy guarantee of the exponential mechanism. However, we chose not to formalize our proof in those terms; instead we provide a self-contained argument leading to a more direct proof without relying on properties of \ac{mDP} established elsewhere.

To start the proof, we first consider the case $\ell = 1$ so that $x = w \in \cW$ and $x' = w' \in \cW$ are two inputs of length one. For any possible output word $\hat{w} \in \cW$ we define a set $C_{\hat{w}} \subset \R^n$ containing all the feature vectors which are closer to the embedding $\phi(\hat{w})$ than to the embedding of any other word. Formally, we have
\begin{align*}
C_{\hat{w}} = \left\{ z \in \R^n \;:\; \norm{z - \phi(\hat{w})} < \min_{u \in \cW \setminus \{\hat{w}\}} \norm{z - \phi(u)} \right\} \enspace.
\end{align*}
The set $C_{\hat{w}}$ is introduced because it is directly related to the probability that the mechanism $M$ on input $x = w$ produces $\hat{w}$ as output. Indeed, by the description of $M$ we see that we get $M(w) = \hat{w}$ if and only if the perturbed feature vector $\hat{\phi} = \phi(w) + N$ is closer to $\phi(\hat{w})$ than to the embedding of any other word in $\cW$. In particular, letting $p_{\phi(w) + N}(z)$ denote the density of the random variable $\phi(w) + N$, we can write the probability of this event as follows:
\begin{align*} % TD: I moved the alignment tab below to stop it going into the margin
\Pr[M(w) &= \hat{w}]
=
\Pr[ \phi(w) + N \in C_{\hat{w}} ]
=
\int_{C_{\hat{w}}} p_{\phi(w) + N}(z) dz \\
&=
\int_{C_{\hat{w}}} p_{N}(z - \phi(w)) dz
\propto
\int_{C_{\hat{w}}} \exp(- \varepsilon \norm{z - \phi(w)}) dz \enspace,
\end{align*}
where we used that $\phi(w) + N$ has exactly the same distribution of $N$ but with a different mean.
Now we note that the triangle inequality for the norm $\norm{\cdot}$ implies that for any $z \in \R^n$ we have the following inequality:
\begin{align*}
\exp(- \varepsilon \norm{z - \phi(w)})
&=
\frac{\exp(- \varepsilon \norm{z - \phi(w)})}{\exp(- \varepsilon \norm{z - \phi(w')})} \exp(- \varepsilon \norm{z - \phi(w')}) \\
&=
\exp(\varepsilon (\norm{z - \phi(w')} - \norm{z - \phi(w)})) \\ 
& \;\; \times \;
\exp(- \varepsilon \norm{z - \phi(w')}) \\
&\leq
\exp(\varepsilon \norm{\phi(w) - \phi(w')} ) \exp(- \varepsilon \norm{z - \phi(w')}) \\
&=
\exp(\varepsilon d(w,w') ) \exp(- \varepsilon \norm{z - \phi(w')}) \enspace.
\end{align*}
Thus, by plugging the last two derivations together and observing the the normalization constants in $p_N(z)$ and $p_{\phi(w) + N}(z)$ are the same, we obtain
\begin{align*}
\frac{\Pr[M(w) = \hat{w}]}{\Pr[M(w') = \hat{w}]}
&=
\frac{\int_{C_{\hat{w}}} \exp(- \varepsilon \norm{z - \phi(w)}) dz}{\int_{C_{\hat{w}}} \exp(- \varepsilon \norm{z - \phi(w')}) dz}
\leq
\exp(\varepsilon d(w,w') ) \enspace.
\end{align*}
Thus, for $\ell = 1$ the mechanism $M$ is $\varepsilon$-mDP.

Now we consider the general case $\ell > 1$. We claim that because the mechanism treats each word in $x = w_1 \cdots w_{\ell}$ independently, the result follows directly from the analysis for the case $\ell = 1$. To see this, we note the following decomposition allows us to write the output distribution of the mechanism on strings of length $\ell > 1$ in terms of the output distributions of the mechanism on strings of length one: for $x, \hat{x} \in \cW^\ell$ we have
\begin{align*}
\Pr[M(x) = \hat{x}] 
&= 
\Pr[M(w_1 \cdots w_{\ell}) = \hat{w}_1 \cdots \hat{w}_{\ell}] \\
&= 
\prod_{i = 1}^\ell \Pr[M(w_i) = \hat{w}_i] \enspace.
\end{align*}
Therefore, using that $M$ is $\varepsilon$-\ac{mDP} with respect to $d$ on strings of length one, we have that for any pair of inputs $x, x' \in \cW^{\ell}$ and any output $\hat{x} \in \cW^{\ell}$ the following is satisfied:
\begin{align*}
\frac{\Pr[M(x) = \hat{x}]}{\Pr[M(x') = \hat{x}]}
&=
\prod_{i = 1}^{\ell} \left(
\frac{Pr[M(w_i) = \hat{w}_i]}{Pr[M(w_i') = \hat{w}_i]}
\right) \\
&
\leq
\prod_{i = 1}^{\ell} \exp(\varepsilon d(w_i,w_i'))
=
\exp(\varepsilon d(x,x')) \enspace,
\end{align*}
where we used that the definition of $d$ is equivalent to $d(x,x') = \sum_{i = 1}^\ell d(w_i,w_i')$. The result follows.

%\section{Analysis of embeddings}
%\input{madlib_appendix1}


\section{Dataset Summary}\label{app:dataset_summary}
\begin{table}[h]
\small
  \caption{Summary of selected dataset properties for IMDb, Enron and InsuranceQA}
  \label{tab:dataset_summary}
\begin{tabular}{lllll}
\toprule
Dataset & IMDb & Enron & InsuranceQA\\
\midrule
Task type & binary  & multi-class  & QA \\
Training set size & $25,000$ & $8,517$ & $12,887$ \\
Test set size & $25,000$ & $850$ & $1,800$ \\
Total word count & $5,958,157$ & $307,639$ & $92,095$ \\
Vocabulary size & $79,428$ & $15,570$ & $2,745$ \\
Sentence length & \makecell[l]{$\mu = 42.27$ \\ $\sigma = 34.38$} & \makecell[l]{$\mu = 30.68$ \\ $\sigma = 31.54$} & \makecell[l]{$\mu = 7.15$ \\ $\sigma = 2.06$} \\
\bottomrule
\end{tabular}
\end{table}



\section{Additional Plausible Deniability Statistics}\label{app:plausible_deniability_fastext}
% \fastextScale output [1200=18, 1600=24, 2000=30, 2400=36, 3000=42]
In this section, we highlight the results of empirical $S_w$ and $N_w$ plausible deniability statistics for $300$ dimension fastText and $50$ dimension GloVe embeddings. The results were designed to yield comparable numbers to those presented for $300$ dimension GloVe embeddings in Figure~\ref{fig:tune-epsilon-glove}

\begin{figure*}
\begin{subfigure}[t]{\textwidth}
    \includegraphics[width=.205\linewidth]{images/eps/fastext_distinct_18}
    \includegraphics[width=.19\linewidth]{images/eps/fastext_distinct_24}
    \includegraphics[width=.19\linewidth]{images/eps/fastext_distinct_30}
    \includegraphics[width=.19\linewidth]{images/eps/fastext_distinct_36}
    \includegraphics[width=.19\linewidth]{images/eps/fastext_distinct_42}
\end{subfigure}
\begin{subfigure}[t]{\textwidth}
    \includegraphics[width=.205\linewidth]{images/eps/fastext_original_18}
    \includegraphics[width=.19\linewidth]{images/eps/fastext_original_24}
    \includegraphics[width=.19\linewidth]{images/eps/fastext_original_30}
    \includegraphics[width=.19\linewidth]{images/eps/fastext_original_36}
    \includegraphics[width=.19\linewidth]{images/eps/fastext_original_42}
\end{subfigure}
\caption{Empirical $S_w$ and $N_w$ statistics for fastText word embeddings as a function of $\varepsilon$.}
\label{fig:tune-epsilon-fastext}
\end{figure*}



\begin{figure*}
\begin{subfigure}[t]{\textwidth}
    \includegraphics[width=.205\linewidth]{images/eps/glove50d_distinct_5}
    \includegraphics[width=.19\linewidth]{images/eps/glove50d_distinct_7}
    \includegraphics[width=.19\linewidth]{images/eps/glove50d_distinct_9}
    \includegraphics[width=.19\linewidth]{images/eps/glove50d_distinct_11}
    \includegraphics[width=.19\linewidth]{images/eps/glove50d_distinct_12}
\end{subfigure}
\begin{subfigure}[t]{\textwidth}
    \includegraphics[width=.205\linewidth]{images/eps/glove50d_original_5}
    \includegraphics[width=.19\linewidth]{images/eps/glove50d_original_7}
    \includegraphics[width=.19\linewidth]{images/eps/glove50d_original_9}
    \includegraphics[width=.19\linewidth]{images/eps/glove50d_original_11}
    \includegraphics[width=.19\linewidth]{images/eps/glove50d_original_12}
\end{subfigure}
\caption{Empirical $S_w$ and $N_w$ statistics for $50$ dimensional GloVe word embeddings as a function of $\varepsilon$.}
\label{fig:tune-epsilon-glove50d}
\end{figure*}



\begin{figure}[h]
\begin{subfigure}[t]{\linewidth}
    \includegraphics[width=.51\linewidth]{images/eps/averageS_w_glove_glove50d}
    \includegraphics[width=.49\linewidth]{images/eps/averageN_w_glove_glove50d}
\end{subfigure}
\caption{Average $S_w$ and $N_w$ statistics for $300$ dimension GloVe embeddings and $50$ dimension GloVe embeddings}
\label{fig:emb_stat_compare}
\end{figure}

\end{appendices}

